Sparse random Fourier features based interatomic potentials for high entropy alloys

Computational modeling of high entropy alloys (HEA) is challenging given the scalability issues of Density functional theory (DFT) and the non-availability of Interatomic potentials (IP) for molecular dynamics simulations (MD). This work presents a computationally efficient IP for modeling complex elemental interactions present in HEAs. The proposed random features-based IP can accurately model melting behaviour along with various process-related defects. The disordering of atoms during the melting process was simulated. Predicted atomic forces are within 0.08 eV/$\unicode{xC5}$ of corresponding DFT forces. MD simulations predictions of mechanical and thermal properties are within 7$\%$ of the DFT values. High-temperature self-diffusion in the alloy system was investigated using the IP. A novel sparse model is also proposed which reduces the computational cost by 94$\%$ without compromising on the force prediction accuracy.

==> OldMelting.tex <==
\subsection{Melting}
\label{sec:melting}
Using the O-RFF potential, we studied the melting behaviour of the FNCCC alloy. An FCC simulations cell of dimension $21.4\AA \times 21.4\AA \times 21.4\AA$ was constructed, and positions were filled randomly with atoms from the design space. We specified the initial velocity distribution corresponding to 300K and raised the temperature till 2500K in discrete steps of 100K. At each step, the simulation box was equilibrated at the corresponding temperature using NPT ensemble. The equilibration at each temperature was performed for 1.2 picoseconds using a time step of 4 femtoseconds. The temperature raise from 300K till 2500K was performed in 27.6 picoseconds. 

%FIGURE 4
\begin{figure}[!ht]
\centering
\includegraphics[trim=-1 0.1 0.1 0.1,clip,scale=0.4]{HEAFigures/HEA-TempVolume.png}

\caption{\label{f:fig4} Variation of volume with respect to temperature as well as percentage of FCC atoms at each temperature are shown in (b). Radial distribution function plots at various temperatures are shown in (b).}
\end{figure}

Figure \ref{f:fig4}(a) shows the variation of average volume with respect to the average temperature for the resulting trajectory. We also performed common neighbour analysis using the Polyhedral matching template algorithm as implemented in OVITO \cite{ovitoRef}. For the entire simulation, we only observed a change in the FCC phase into other phases. Figure \ref{f:fig4}(a) also shows the percentage of FCC atoms corresponding to each temperature.  As expected, with an increase in temperature, an increase in volume and a decrease in the crystal symmetry are observed. 

The radial distribution function (RDF) of the FNCCC alloy at various temperatures is also shown in Figure \ref{f:fig4}(b). At 300K, there are sharp peaks at first and second neighbour distances, indicating FCC symmetry. Raising the temperature to 900K reduces the peak height and increases the curve width. From Figure \ref{f:fig4}(a), we can see that this is the temperature where the FCC phase starts converting into other phases. The percentage of FCC atoms continues to decline steadily, and a sharp drop is observed starting at 1500K but not much change in the slope of the temperature-volume curve is observed. Further, another sharp drop is observed between 1600K – 1700K and a slight change in the slope of the temperature-volume curve is also noticed, indicating the melting process has started. At 1700K, only 10\% of the atoms are in FCC state which steadily goes to zero at 2000K. RDF plots are showing similar density beyond 1700K. Also, we noticed a sharp change in slope in the temperature-volume curve at 1700K. From these observations, we conclude that the melting temperature for FNCCC should lie in the range of 1500 - 2000K. Experimentally, the melting temperature of this alloy is found to be 1500K \cite{meltFNCCC}, which further corroborate our observation regarding the melting temperature. 

\subsection{Diffusion Coefficients}
The coefficient of self-diffusion was calculated for each species using the O-RFF potentials. Self-diffusion constants ($D_{self}$) can be calculated from the asymptotic behavior of the mean-square displacement (MSD) of atoms as follows
%Add text here
\begin{equation}
    \label{e:diff_eq}
    D_{self} = \frac{1}{6} \lim_{t\to\infty} \frac{d (MSD)}{dt}.
\end{equation}
For a particular temperature of interest, the MSD of the atoms can be extracted from the MD trajectory using the following equation known as the Einstein formula

\begin{equation}
    \label{e:msd}
    MSD = \Bigg \langle \frac{1}{N_{atoms}} \sum_{n=1}^{N_{atoms}} \vert r_{\alpha}^{n} - r_{\alpha}^{n}(t_0) \vert^2 \Bigg \rangle_{t_{0}},
\end{equation}
where $N_{atoms}$ is the number of atoms in the system and $r_{\alpha}^{n}$ are their coordinates which are averaged over time origins \cite{mei1990molecular, maginn2019best}.

Figure \ref{f:fig_diff}(a) shows the MSD of Cobalt in the FNCCC within the temperature range 1500K - 2300K. The MSD at lower temperatures have a linear region followed by a steady plateau. This is typical behavior of solid state materials \cite{chen2013melting}. As the temperature increases, this plateau gradually disappears ( \(\sim\)1900K-2000K). MSD becomes a straight line with a single slope from 2100K onward indicating the complete transformation of the FNCCC to liquid state. This is in agreement with the evolution of crystalline ordering observed during the melting process as discussed in \ref{sec:melting}. MSD for other component species follows the same trend as this. Calculated diffusion constant values from the MSD are plotted in Figure \ref{f:fig_diff}(b).  The absolute values of self-diffusion constants are of the same order of magnitude as reported in the literature \cite{neumann2011selfdiffusion}. This suggests that the O-RFF potential can be reliably used to perform calculations at elevated temperatures where the diffusive mechanisms are dominant.

%FIGURE 5
\begin{figure}[!ht]
\centering
\includegraphics[trim=-1 0.1 0.1 0.1,clip,scale=0.35]{HEAFigures/diffusion_compiled.jpg}

\caption{\label{f:fig_diff} (a) Mean Square Displacement as a function of simulation time for Cobalt in FNCCC (b) Self-diffusion constants for each species in the alloy}
\end{figure}


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


